Pay Attention to the Atlas: Atlas-Guided Test-Time Adaptation Method for Robust 3D Medical Image Segmentation

Convolutional neural networks (CNNs) often suffer from poor performance when tested on target data that differs from the training (source) data distribution, particularly in medical imaging applications where variations in imaging protocols across different clinical sites and scanners lead to different imaging appearances. However, re-accessing source training data for unsupervised domain adaptation or labeling additional test data for model fine-tuning can be difficult due to privacy issues and high labeling costs, respectively. To solve this problem, we propose a novel atlas-guided test-time adaptation (TTA) method for robust 3D medical image segmentation, called AdaAtlas. AdaAtlas only takes one single unlabeled test sample as input and adapts the segmentation network by minimizing an atlas-based loss. Specifically, the network is adapted so that its prediction after registration is aligned with the learned atlas in the atlas space, which helps to reduce anatomical segmentation errors at test time. In addition, different from most existing TTA methods which restrict the adaptation to batch normalization blocks in the segmentation network only, we further exploit the use of channel and spatial attention blocks for improved adaptability at test time. Extensive experiments on multiple datasets from different sites show that AdaAtlas with attention blocks adapted (AdaAtlas-Attention) achieves superior performance improvements, greatly outperforming other competitive TTA methods.

==> novelty_statement.tex <==
% Statement of Novelty/Impact: This statement, of up to 500 characters in length, should provide the main argument for the inclusion of the paper in the conference. It should clarify whether the main significance of the contribution is in the novelty of the proposed methodology or the scientific/clinical impact of the conclusions or results. Note that this statement will be visible to reviewers and area chairs and should not identify the authors or their institutions.

%% 500 char.
 We present a novel atlas-guided test-time adaptation (TTA) framework for robust 3D medical image segmentation on unseen domains, which greatly outperforms competitive TTA methods by a large margin. Particularly, we revolutionize the use of attention blocks for TTA and our study unveils the importance of building flexibility into the design of network architecture as well as constructing reliable supervision signals at test-time adaptation. 

==> todo.tex <==
% 1. change Figure 1 with an explanatory figure. move D to supplementary.
% 2. Equation 5, add under brackets if space allows
% 3. Table 1, simply, put detailed one into supplementary.
% 4. add limitations
5. conduct p-value test
6. provide data links in the reference

